Rule-based Modelling and Tunable Resolution

We investigate the use of an extension of rule-based modelling for cellular signalling to create a structured space of model variants. This enables the incremental development of rule sets that start from simple mechanisms and which, by a gradual increase in agent and rule resolution, evolve into more detailed descriptions.

==> eptcsdata.tex <==
\providecommand{\event}{S. Barry Cooper \& Vincent Danos (eds.): Fifth Workshop on\\
Developments in Computational Models---Computational Models From Nature}
\providecommand{\volume}{9}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{65}
\providecommand{\eid}{8}

